Quantifying uncertainty in spikes estimated from calcium imaging data

In recent years, a number of methods have been proposed to estimate the times at which a neuron spikes on the basis of calcium imaging data. However, quantifying the uncertainty associated with these estimated spikes remains an open problem. We consider a simple and well-studied model for calcium imaging data, which states that calcium decays exponentially in the absence of a spike, and instantaneously increases when a spike occurs. We wish to test the null hypothesis that the neuron did not spike -- i.e., that there was no increase in calcium -- at a particular timepoint at which a spike was estimated. In this setting, classical hypothesis tests lead to inflated Type I error, because the spike was estimated on the same data used for testing. To overcome this problem, we propose a selective inference approach. We describe an efficient algorithm to compute finite-sample p-values that control selective Type I error, and confidence intervals with correct selective coverage, for spikes estimated using a recent proposal from the literature. We apply our proposal in simulation and on calcium imaging data from the spikefinder challenge.

==> abstract.tex <==
%!TEX root = ./paper_biostat_revision.tex

In the past few years, a number of methods have been proposed to estimate the times at which a neuron spikes on the basis of calcium imaging data. However,  quantifying the uncertainty associated with these  estimated spikes remains an open problem. 

We consider a simple and well-studied model for calcium imaging data which states that calcium decays exponentially in the absence of a spike, and instantaneously increases when a spike occurs. 
We wish to test the null hypothesis that the neuron did \emph{not} spike --- i.e., there was no increase in calcium --- at a particular timepoint at which a spike was estimated.
 In this setting, classical hypothesis tests lead to inflated Type I error rate because the spike was estimated on the same data used for testing. To overcome this problem, 
 we propose a selective inference approach.  We describe an efficient algorithm to compute finite-sample $p$-values that control selective Type I error, and confidence intervals with correct selective coverage, for spikes estimated using a recent proposal from the literature.  We illustrate the proposed approach in a simulation study and on calcium imaging datasets released as a part of the \texttt{spikefinder} challenge.
